Zero-Shot On-the-Fly Event Schema Induction

What are the events involved in a pandemic outbreak? What steps should be taken when planning a wedding? The answers to these questions can be found by collecting many documents on the complex event of interest, extracting relevant information, and analyzing it. We present a new approach in which large language models are utilized to generate source documents that allow predicting, given a high-level event definition, the specific events, arguments, and relations between them to construct a schema that describes the complex event in its entirety. Using our model, complete schemas on any topic can be generated on-the-fly without any manual data collection, i.e., in a zero-shot manner. Moreover, we develop efficient methods to extract pertinent information from texts and demonstrate in a series of experiments that these schemas are considered to be more complete than human-curated ones in the majority of examined scenarios. Finally, we show that this framework is comparable in performance with previous supervised schema induction methods that rely on collecting real texts while being more general and flexible without the need for a predefined ontology.

==> 07_results.tex <==
\section{Results}
\label{07_results}



==> figures/direct_event.tex <==
\begin{figure}[]
\centering
 \fbox{%
    \parbox{\columnwidth}{%
\textbf{Prompt}: What are the steps involved in holding a summit meeting?

\textbf{Output}:
\begin{enumerate}
    \item \hl{Plan} the agenda and objectives of the meeting.
    \item \hl{Select a venue} that is appropriate for the meeting's purpose and size.
    \item \hl{Send out invitations} and \hl{ensure} all participants have the appropriate information.
    \item \hl{Prepare} for the meeting by \hl{creating materials} and \hl{briefing} the participants.
    \item \hl{Hold} the meeting and \hl{follow up} on any action items that are generated. 
\end{enumerate}
}}
    \caption{Example of generation of steps involved in the event of holding a summit meeting.}
    \label{fig:direct_event2}
\end{figure}

==> figures/model.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/zero-shot.png}
    \caption{something.Bold arrows - processing data into event graphs (event extraction, argument extraction, relation extraction}.
    \label{fig:model}
\end{figure*}

==> figures/news_event.tex <==
% \begin{figure}[]
% \small
%     \centering
%     \fbox{%
%     \parbox{\columnwidth}{%
% \textbf{First prompt}: Write a news headline about winning an Olympic medal

% \textbf{Output}: \textbf{Write a news headline about winning an Olympic medal}. The headline of the news about winning an Olympic medal reads \hl{"The United States won gold in women's water polo"}. I'm not sure about the spelling of the word "won" here, but the fact is: the United States won gold in women's water polo. The US Women's Water Polo Team won the gold medal in the 2008 Beijing Olympics in front of a roaring crowd. A big smile spreads across my face as I type those two sentences. It doesn't seem possible for a few days that the United States won something. But we won. So, who are these ladies and what did they do?

% \textbf{Second prompt}: Write a news story titled: "The United States won gold in women's water polo"

% \textbf{Output}: \textbf{The \hl{United States won gold} in women's water polo at the Summer Olympics} with a \hl{scoreless game in the final} against Spain on Monday.
% \hl{The Americans defeated} China 3-0 \hl{in the semifinals}. The top four teams in each half of the 12-team competition advanced to Sunday's final.
% Japan's silver was a loss to the United States in the quarterfinals, and China's bronze came on a 3-0 victory over Croatia.
% The Americans won their first water polo medal since 2004, and the nation's first since the Summer Olympics returned to the United States.
% %\textbf{Conclusions}: from this we can conclude, for example, that in order to win an Olympic medal, one has to with the finals and the semifinals.
%     }
% }
%     \caption{Example of generation of news-like text for the event of winning an Olympic medal.}
%     \label{fig:news_event}
% \end{figure}

\begin{figure}
    \centering
    \fbox{%
    \parbox{\columnwidth}{%
    %\textbf{First prompt}: Write a news headline about Election.
    \textbf{First prompt}: Write a news headline about filing a patent.
    
    \textbf{Output}: New Patent Filing Could Speed Up Drug Development.
    
    %\textbf{Second prompt}: Write a news story titled: "Bernie Sanders conceded defeat to Hillary Clinton in New Jersey's Democratic primary, even though the state's election results were incomplete."
    \textbf{Second prompt}: Write a news story titled "New Patent Filing Could Speed Up Drug Development".
    
    \textbf{Output}: The United States Patent and Trademark Office has just \hl{published} a new patent that could speed up the drug development process. The patent, \hl{filed by} a team of researchers from the DPharm Institute, \hl{covers} a new drug screening process that could help \hl{identify} potential new drugs much more quickly. The new process, which is based on a computer algorithm, is said to be up to 10 times faster than traditional methods. It can identify potential new drugs by \hl{screening} through large databases of existing drugs and drug candidates. The DPharm Institute is already in the process of \hl{licensing the patent} to several pharmaceutical companies, and is planning to \hl{commercialize the technology} over the next few years.
    %\textbf{Output}: \textbf{Bernie Sanders conceded defeat to Hillary Clinton in New Jersey's Democratic primary, even though the state's election results were incomplete.} 
    %New Jersey's presidential primary was not a typical one. More than one-third of the state's registered voters were \hl{ineligible to vote} because they were \hl{unaffiliated with a party}. And the number of unaffiliated declined since the last presidential primary in 2008 and it's dropping further. Yet, even though more than 1 million unaffiliated voters were not allowed to \hl{cast ballots} this year, the \hl{state's primary was counted} and \hl{declared} while knowing that \hl{Hillary Clinton would win} because she had won the same primary in 2008. With 1.4 million unaffiliated voters, Clinton beat Barack Obama in New Jersey by 1.1 million votes. "Usually -- you don't decide elections while the votes are still being counted," said Steve Kornacki, political analyst at NBC News. "Everything we did that night and that day did not just defy logic and did not just defy precedent and did not just defy tradition, did not just defy previous practice, we did all that we did we did just to just to help Hillary Clinton," said David Birdsell, dean of the Baruch College School of Public Affairs.
    }
    }
    \caption{Example of generation of news-like text for the event of Election.}
    \label{fig:news_event2}
\end{figure}

==> figures/not_news_event.tex <==
\begin{figure}[]
\centering
 \fbox{%
    \parbox{\columnwidth}{%
%\textbf{Prompt}: How to get a Ph.D. degree?
\textbf{Prompt}: Describe how to 3D print an object?
%\textbf{Output}: \textbf{How to get a Ph.D. degree?} It’s complicated. And expensive.

\textbf{Output}: To 3D print an object, you need to first \hl{design the object} in a 3D modeling program. Once the object is designed, you need to \hl{export} it as a 3D printable file format. Next, you need to \hl{choose} a 3D printer and print settings. Finally, you need to \hl{print} the object.
%Getting a Ph.D. is a long and expensive process, with an average completion time of 12-15 years. In the meantime, you can \hl{spend all that time and money} (and you will have to) without a degree, but you will have a heck of a time \hl{finding a tenure-track position}. And there’s the cost. So, here are the facts: Ph.D.s are very, very hard to get. I mean hard to get in the sense that there are so few. And hard to get in the sense that you will have to work really, really hard and spend years, and years, and years to get one. There is a lot of competition for them, and there are very few places you can study. You will \hl{have to be an outstanding student} and \hl{get really good grades in graduate school} to have a chance of winning a spot in a very competitive doctoral program. The competition is really stiff. \hl{Getting into one of the top schools} that you will need to get into is very competitive.
}}
    \caption{Example of generation of text of how-to.}
    \label{fig:not_news_event2}
\end{figure}

==> unrelated_ignore.tex <==
Goal: train a language model that will be aware of events in a sentence, the event arguments and the relations between different events.



\section{Relevant works}
\begin{itemize}
    \item \cite{li2020connecting} - Connecting the Dots: Event Graph Schema Induction with Path Language Modeling. Path Language Model, an auto-regressive language model trained on event-event paths, and select salient and coherent paths to probabilistically construct these graph schemas. link: \url{https://www.aclweb.org/anthology/2020.emnlp-main.50.pdf}
    \item \cite{fei2020enriching} - Enriching contextualized language model from knowledge graph for biomedical information extraction. propose to enrich a contextualized language model by integrating a large scale of biomedical knowledge graphs (namely, BioKGLM). In order to effectively encode knowledge, we explore a three-stage training procedure and introduce different fusion strategies to facilitate knowledge injection. link: \url{https://academic.oup.com/bib/advance-article/doi/10.1093/bib/bbaa110/5854405}
    \item Med-BERT: pre-trained contextualized embeddings on large-scale structured electronic health records for disease. Objective: To investigate whether pre-trained contextualized embeddings on large-scale structured EHRs can benefit downstream disease-prediction tasks and to share the pre-trained model and relevant tools with the public. link: \url{https://arxiv.org/pdf/2005.12833.pdf}
    \item \cite{alon2020structural} Structural Language Models of Code.We present a new approach that explicitly models the source and the target code as the same tree – structural language modeling (SLM). SLM estimates the probability of the program’s abstract syntax tree (AST) by decomposing it into a product of conditional probabilities over its nodes. We present a neural model that computes these conditional probabilities by considering all AST paths leading to a target node, generalizing over traditional language models that consider sequences of words. While prior work uses AST paths to read programs (Alon et al., 2019b), we generate code by predicting the next node along the set of paths, generating the target AST node-by-node. link: \url{https://arxiv.org/pdf/1910.00577.pdf}
    \item 
    
1. IED Bombing

2. Pandemic/Disease Outbreak

3. Civil Unrest

4. International Conflict

5. Disaster and Rescue

6. Terrorism Attacks

7. Election

8. Sports Games

9. Kidnapping

10. Business Change
\end{itemize}

\section{Data}

\section{Evaluation}
\begin{itemize}
    \item Event schema induction
    \item ROC Story Cloze Task \cite{mostafazadeh2016corpus}
    \item Question answering about timeline - TORQUE dataset \cite{ning2020torque}.
    \item Predicting NER and event relations.
\end{itemize}
